Shard Scheduler: object placement and migration in sharded account-based blockchains

We propose Shard Scheduler, a system for object placement and migration in account-based sharded blockchains. Our system calculates optimal placement and decides of object migrations across shards and supports complex multi-account transactions caused by smart contracts. Placement and migration decisions made by Shard Scheduler are fully deterministic, verifiable, and can be made part of the consensus protocol. Shard Scheduler reduces the number of costly cross-shard transactions, ensures balanced load distribution and maximizes the number of processed transactions for the blockchain as a whole. It leverages a novel incentive model motivating miners to maximize the global throughput of the entire blockchain rather than the throughput of a specific shard. Shard Scheduler reduces the number of costly cross-shard transactions by half in our simulations, ensuring equal load and increasing the throughput 3 fold when using 60 shards. We also implement and evaluate Shard Scheduler on Chainspace, more than doubling its throughput and reducing user-perceived latency by 70% when using 10 shards.

==> sections/analysis.tex <==
%!TEX root = ../main.tex
%=========================================================

\section{Analysis and discussion}
\label{sec:analysis}
We start by analyzing the security of \sysname against the properties defined in \Cref{sec:design_goals}. We discuss next implementation consideration. 

\michal{Goals: equal load, limited number of migrations, }


\subsection{Achievement of Design Goals}

\para{Migration and placement recommendations}

\para{Recommendation verifiability} 
load + allignments, based on blockchain

Main shard is chosen by one of the shard

\para{Lightweight}

\para{No changes for the clients}

\para{Incentive model}



==> sections/analytics.tex <==
%!TEX root = ../main.tex
%=========================================================

\section{Analytics}

\subsection{Users and Transactions}
We start by analyzing the number of users and their activity in the network. \Cref{fig:ethereum_cdf} presents a CDF of users in terms of number of transactions they were involved in. The vast majority (80\%) of users were involved in 1-3 transactions.\mustafa{How do you define a "user"? There's no conception of a user on a blockchain. Only addresses. Did you de-anonymise everyone and manage to cluster addresses to individual users? :-)} On the other hand, there are few extremely active nodes (usually exchanges and mining polls) responsible for the majority of transactions. The orange line shows the percentage of transactions users with given amount of transactions were involved in. We can see, that the least active users (who were involved in 1 transaction only) are responsible for $\sim$4\% of the traffic). We can also observe few large players being observed by more than 20\% of the transactions. 

\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_cdf_transactions}
\caption{CDF of users with given number of transactions}
\label{fig:ethereum_cdf_transactions}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_cdf_peers}
\caption{CDF of users with given number of peers they interact with}
\label{fig:ethereum_cdf_peers}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_cdf_weights}
\caption{CDF of edges with given weight. A weight of 2 means that users interacted 2 times.}
\label{fig:ethereum_cdf_weights}
\end{figure}

This inequality in users' activity causes problems when thinking about sharding state based on hashes of user addresses. While user addresses are spread uniformly among the hash space, the number of transaction is not (\Cref{fig:ethereum_tx_user_shards_10}). Shards with active users experience much higher load than other shards. This problem becomes even more pronounced when the number of shards increases (\Cref{fig:ethereum_tx_user_shards_10}).


\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_tx_user_shards_10}
\caption{Number of users and transactions assigned for each out of 10 shards.}
\label{fig:ethereum_tx_user_shards_10}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_tx_user_shards_100}
\caption{Number of users and transactions assigned for each out of 100 shards.}
\label{fig:ethereum_tx_user_shards_100}
\end{figure}

Those results show that it's important to mix active and inactive users and achieve balance among shards in terms of both the number of users and the number of transactions.

\subsection{Blockchain activity over time/Transactions type}
We analyse the number of transaction performed in 100/1000/10000 blocks (\Cref{fig:ethereum_activity_100}, \Cref{fig:ethereum_activity_1000}, \Cref{fig:ethereum_activity_10000}). The graphs show a clear increasing trend in the blockchain activity. At the same time, within the trend, we observe severe fluctuation in the number of transactions. In Ethereum, each new block is generated every ~12s. It means that 100 blocks = 20min, 1000 blocks = 3.3h, 10000 = 33h.

\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_activity_100}
\caption{Number of transactions per 100 blocks.}
\label{fig:ethereum_activity_100}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_activity_1000}
\caption{Number of transactions per 1000 blocks.}
\label{fig:ethereum_activity_1000}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_activity_10000}
\caption{Number of transactions per 10000 blocks.}
\label{fig:ethereum_activity_10000}
\end{figure}

Furthermore, we analyze types of transactions. We distinguish between:
\begin{itemize}
 \item new\_new - a transaction between two addresses that have not been previously seen in the ledger.
 \item old\_new - a transaction between an address that have been previously seen in the ledger and one that have not been seen.
 \item old\_old - a transaction between two addresses that have been previously seen in the ledger.
\end{itemize}

\Cref{fig:ethereum_transactions_1000}, \Cref{fig:ethereum_transactions_10000} and \Cref{fig:ethereum_transactions_100000} present the number of transactions of each type in a batch of 1000, 10000 and 100000 transactions respectively. The vast majority of transactions concist of old\_old type. Suggesting that optimal placements of highly communicating users can bring a lot of benefits in terms of performance.


\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_transactions_1000}
\caption{Type of transactions per 1000 transactions.}
\label{fig:ethereum_transactions_1000}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_transactions_10000}
\caption{Type of transactions per 10000 transactions.}
\label{fig:ethereum_transactions_10000}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/ethereum_transactions_100000}
\caption{Type of transactions per 100000 transactions.}
\label{fig:ethereum_transactions_100000}
\end{figure}


\subsection{TODO}
\begin{itemize}
 \item CDF - with how many users you interact (global)
 \item CDF - what's the max(?) number of time you interact with the same users (global)
 \item CDF - how many time you interact with each of your peer (local)
\end{itemize}

Extract characteristics:
\begin{itemize}
 \item how many
\end{itemize}


==> sections/problem.tex <==
%!TEX root = ../main.tex
%=========================================================

\section{Problem formulation}
\label{sec:problem}

\subsection{Blockchain/Ethereum}
The blockchain is a replicated state machine. It consists of a set of state variables that encode its state $s \in S$ and transactions $t \in T$. The blockchain maintains an append-only log of ordered transactions $\{t_0...t_n\} \in T$. The blockchain starts in an initial state $t_0 \in T$ and transition from one valid state to the valid next state with each valid transaction $t_i(s_i) \rightarrow s_{i+1}$. Each transaction is executed deterministically (that is, transactions are atomic). \mustafa{Nitpick: a blockchain is just a chain of blocks, used to create an append-only DB. You can use it to build a state machine. See LazyLedger for example.}\mustafa{Isn't the initial state $s_0$ not $t_0$?}

Ethereum is an account-based blockchain. It means that the ledger stores monetary transactions between users $u \in U$. Each transaction  has a sender, a receiver and an amount $t_i: (from \in U, to \in U, amount)$. Each state represents balances of all the users $b \in B$ where $b_i$ is the balance of users $u_i$. Thus state at interval $i$ consists of $s_i: \{b_0,...,b_n\}$. A transaction from user 1 to user 2 with an amount of x $t_k: (u_1, u_2, x)$, modify the state $s_i$ (if the sender have enough money to perform the transaction), so that in $s_{i+1}: b_1 \leftarrow b_1 - x, (b_1 \ge x) \land b_2 \leftarrow b_2 + x$. If the sender does not have enough money to perform the transaction, the transaction is invalid and should be discarder.\mustafa{The state in Ethereum consists of a lot more than balances. It consists of a key=>value store, that smart contracts can modify, as each smart contract can define variables and store data. Are you pretending that there is only balances in the state for your model and ignoring smart contracts? If so then that's important to mention.}

The blockchain is maintained by miners $m \in M$, who validate and exchange the transactions; and agree on a global transaction order using a consensus protocol.
\michal{probably need to introduce mining power here}
To perform their tasks, every single miner is required to replicate (Network I/O Bound), validate (CPU Bound) and store (Disk I/O Bound) all transactions. Every single miner is required to maintain states (Memory Bound) of all users in entire network. Such an approach limits the number of transactions that can be processed by the network.

This is why sharding was introduced, where the blockchain is divides into groups called shards(zones) $z \in Z$. Each shard maintaines a subset of the state and thus balances of a subset of the users ($U_j: {u_i,...,u_k}$ so that  ${b_i,...,b_k} \in z_j$). So that shard $z_j$ at step $i$ maintains $s_{ij}: b_k \forall u_k \in U_j$. Miners in a shard requires now to process only transactions modifying state of users in the same shard and not all the users. In general, this approach allows to increase the number of transactions per second (TPS) when increasing the number of shards.

With sharded blockchains, we distinguish between 2 types of transactions:
\begin{itemize}
 \item intra-shard - $t_{\textit{intra}}: (u_1, u_2, x)$, where $u_1, u_2 \in U_i$
 \item inter-shard - $t_{\textit{inter}}: (u_1, u_2, x)$, where $u_1 \in U_i, u_2 \in U_j, i \ne j $
\end{itemize}

Intra-shard transaction are simple and relatively cheap as they require only agreeing within one shard. In contrast, inter-shard transactions require processing a transaction in two shards as well as making those transactions atomic (either both are executed or none). This imply inter-shard communication.

$s_{\textit{inter}}: b_1 \leftarrow b_1 - x, (b_1 \ge x) \in z_{i} \land b_2 \leftarrow b_2 + x \in z_{j}$

\mustafa{Hmm we need to be careful here because again this is ignoring the fact that Ethereum is a general purpose smart contract platform, not a payment platform. Technically inter-shard transactions are defined as when a smart contract in one shard accesses state in a different shard. You could argue the payment case is a subset of that generalisation.}
\mustafa{Also why is the paper only considering txes that involve 2 shards? What about more than 2 shards? There could be inputs from 3 shards for example}

\michal{With increased complexity of inter-shard transaction comes higher cost for the users. So users are naturally incentivized to minimize the number of inter-shard transactions. We could use this mechanism and provide an off-chain oracle that user can use to get the optimal placement, but users don't have to obey.}

\michal{Random thought: what if each user automatically has a subcount for each shard -  <user\_addr>@<shard\_id> with seperate balances. Maybe it would be enough to drastically minimize the number of inter-shard transactions. You only have to perform inter-shard transactions if you don't have enough funds in a specific shard. Probably users rarely spend all their money at once, so the money could be split into sub-accounts. \mustafa{Big exchanges and company will likely do this for sure.}}


\subsubsection{Assigning state to shards}
State sharding is usually done based on user addresses (the address is hashed and assigned to a shard) \hl{refs needed}. A transaction will be processed by the shard responsible for keeping sender's state.
\michal{put more info} \mustafa{Hmm I'm not sure, and this raises in interesting question as I'm not sure how defined this is yet in Eth 2. I don't see any reason why the same address couldn't exist in every shard for example. I'll ask around..}

\subsubsection{Mining power}
As mentioned before, blockchains require consensus to agree on transaction order. However, consensus must be run between identities. This is difficult, as miners can create multiple Sybil (fake) identities online. To solve this problem, a concept of mining power was introduced. Each miner's voting power when reaching a consensus is bound to its mining power divided by the total mining power of all the miners. The system is safe as long as honest miner control 50\% or 66\% (depending on the consensus protocol) of the total mining power. The most popular system binds user mining power to physical resources (CPU hashrate in Proof of Work (PoW)) or the amount of money they have in the system (Proof of Stake (PoS)).

When dividing a blockchain into shards, we must make sure that in each shard there's an honest majority (in terms of mining power).\mustafa{I don't think you need too much detail here because the cross-chain protocol is generally independent of the underlying consensus protocol.}

\michal{We could also optimize the assignment of miners to shards. Also users with high mining power, could be validators in multiple shards. If that's the case, we should assign them to shards that communicate often. Like that we minimize the cost of inter-shards transactions. \mustafa{Why would that minimise the cost of inter-shard transactions? Worth thinking about full nodes in shards too verifying the chain for themselves.}}


\subsection{Problem formulation}
An undirected weighted graph is $G = (V,E)$ where each edge $e \in V \times V$.
The edge weight is denoted $w(e) \in \mathbb{N}^+$.
We also denote the the weight of a set of edges as $w(\{e_1,...,e_m\}) = \sum_{i=1}^m w(e_i)$.

We refer to the following problem as the Weighted k-Way Graph Partitioning (GP).


Given an undirected graph $G$ and an integer $B$, partition the vertices $V$ into subsets, called clusters or shards
$C_1,C_2,\ldots, C_k$ such that each $C_i$ has at most $B$ vertices and the number of inter-cluster edges is minimized, i.e.,
minimize $w(cut({C_1,...,C_k}))$ where $cut({C_1,...,C_k}) = \{ e=(u,v) \mid u \in C_i \wedge v \in C_j \ \mathrm{where} \ i \neq j \}$.

In the offline version, it is assumed that the entire graph and weights is known to the algorithm in the beginning.

In the online version of this problem we consider the weights are an increasing function over time.
We denote weight of edge $e$ at time $t$ as $w_t(e)$ with $t \in [0..n]$.
Initially all the weights are null $w_0(e) = 0,  \forall e$.
Then at every time $t \in [1..n]$, the weight of exactly one edge $e$ is incremented:
$w_t(e) \leftarrow w_{t-1}(e)+1$ and $w_t(e')= w_{t-1}(e'), \forall e' \neq e$.
The stream of edges inducing a modification of the weights is $[e_1,e_2,\ldots,e_n]$.

TODO: explain the decision that we need to take in the online-version.


\subsection{Problem formulation2}\label{sec:problem2}
We have:
\begin{itemize}
 \item discrete time
 \item a global history of transactions $\mathcal{H}$.
 \item an input buffer of transactions to be processed $\mathcal{I}$ with the size of $s_{\mathcal{I}}$
 \item a fixed number of $n$ shards $\mathcal{Z} = \{z_0,...z_n\}$
 \item Each shard has a fixed processing capacity of $C_z$ per time step
 \item a mapping of users to shards $\mathcal{M} = \{u_0 \rightarrow z_i,...,u_n \rightarrow z_j\}$
\end{itemize}

At each time step:
\begin{itemize}
 \item $\mathcal{I}$ is filled with transactions from $\mathcal{H}$ up to its maximum size $s_{\mathcal{I}}$
 \item Each current shard's capacity is set to $\forall i, c_i = C_z$
 \item We iterate through transactions in $\mathcal{I}$, each transaction happens between 2 users $u_1 \rightarrow u_2$
 \item We have 2 types of transactions:
 \begin{itemize}
    \item intra-shard - $t_{\textit{intra}}: (u_1, u_2, x)$, where $\mathcal{M}(u_1) = \mathcal{M}(u_2) = z_i$
    \item inter-shard - $t_{\textit{inter}}: (u_1, u_2, x)$, where $\mathcal{M}(u_1) = z_i, \mathcal{M}(u_2) = z_j, i \ne j $
 \end{itemize}
 \item An intra-shard transaction can be processed if current capacity of $z_i$ is at least 1 $c_i \ge 1$. If it's the case, the current capacity is lowered by 1 $c_i = c_i - 1$, and the transaction is removed from $\mathcal{I}$.
 \item An inter-shard transaction can be processed if current capacity of both shards is at least 1.5  $z_i \ge 1.5$ and $z_i \ge 1.5$. If it's the case, the current capacity is of both shards is lowered by 1.5 $c_i = c_i - 1.5, c_j = c_j - 1.5$ and the transaction is removed from $\mathcal{I}$.\mustafa{Why 1.5, shouldn't it be 2? What about inter-shard txes involves more than 2 shards BTW?}
 \item If some transactions cannot be processed, they stay in $\mathcal{I}$ for future iterations.
 \item At the end of each iteration, we can decide to modify $\mathcal{M}$ and move users between shards. State migration of user $u_i$ from shard $z_j$ to shard $z_k$ is equivalnt to an inter-shrard transaction between both shards (with an equal cost 1.5 in both shards), is added to $\mathcal{I}$ and will be executed during future iterations.
\end{itemize}

The goal is to minimize the number of time steps required to process all the transactions from $\mathcal{H}$.


\michal{Make 2 passes - first intra-shard transactions only, then inter-shard transactions}


==> sections/propositions.tex <==
%!TEX root = ../main.tex
%=========================================================

\section{Proposed solutions}

In this section, we propose and evaluate some solutions to optimally divide state.
We build a Python simulator replaying Ethereum history of transactions using problem formulation presented in \Cref{sec:problem2}. 

We define following policies:
\begin{itemize}
 \item Random/Hash-based - users are assigned to shard based on the hash of their addresses. 
 \item Louvain Policy - We create an interaction graph using the whole transaction history. We then detect highly communicating communities using the Louvain Method~\cite{blondel2008fast}. If the method creates more communities than shard (it's usually the case), we assign communities to shards using First Fit Decreasing algorithm. The size of each community is calculated based on the sum of edge weights and translates into a total number of transactions performed by each community. This allows us to keep roughly the same number of transactions per shard. 
 \item SameAsFirst - if both user involved in a transaction are seen for the first time, we put them together in a random shard. If one of them is already assigned, we put the other on in the same shard. If both addresses are already assigned, we don't move them. 
 \item Louvain+SameAsFirst - We use 50\% of the history as with the Louvain policy. For the rest we use the SameAsFirst policy. 
\end{itemize}


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/policy_s10_b1000}
        \caption[Network2]%
        {{\small Network 1}}    
        \label{fig:mean and std of net14}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.495\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{img/policy_s10_b10000}
        \caption[]%
        {{\small Network 2}}    
        \label{fig:mean and std of net24}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.485\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{img/policy_s100_b10000}
        \caption[]%
        {{\small Network 3}}    
        \label{fig:mean and std of net34}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.485\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{img/policy_s100_b100000}
        \caption[]%
        {{\small Network 4}}    
        \label{fig:mean and std of net44}
    \end{subfigure}
    \caption[ The average and standard deviation of critical parameters ]
    {\small The average and standard deviation of critical parameters: Region R4} 
    \label{fig:mean and std of nets}
\end{figure*}


\michal{calculate what's the probability that the next transaction would be with the most frequently contacted node. See if they communicate in bursts with one users, or keep constant, frequent relations.}

\michal{Maybe we could use fading edges? If it was added a long time ago - remove it}

\michal{In DHTs, one usually tries to stick to active peers that they had relations with for the longest time. Maybe we should try having a similar approach here? A node will be marked as inactive if there was no transaction during last X blocks. However, we try to keep each addr with the same shard as their oldest active friends.}
% \subsection{Naive solution}
% We assume that the distribution of state among shards will happen on already existing history of the ledger. We could thus perform an initial distribution using the Louvain method and thus simply assign new users to the same shard as the sender, who first sent them a transaction. If a user appears after mining coins, they will be assigned to a random shard. 
% 
% To evaluate this approach, we divide Ethereum ledger in half. After 50\% of transactions, we split users into group using the Louvain method, we then assign new users as described above (partial). We compare this solution against a ``full'' solution where we run the Louvain method for the full ledger history. \Cref{fig:ethereum_naive} presents the results. The number of inter-shard transactions increases quickly for the partial solution, but then expieriences similar increase as the full solution. Note, that the graph shows inter-group connections, not inter-shard connections. The louvain method produces a number of groups much higher than the number of shards. The groups must be then assigned to shards. 
% 
% 
% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.45]{img/ethereum_naive}
% \caption{Number of inter/intra-shard connections for a full and a partial solution.}
% \label{fig:ethereum_naive}
% \end{figure}


\subsection{DB-inspired approach}
This is directly inspired by Clay~\cite{serafini2016clay}. At each interval we iterate through all the nodes that have been active (involved in a transaction) in the overloaded (or highly loaded shards). For each node, we iterate through all its edges and calculate if moving to a different (less loaded) shard would reduce the number of inter-shard transactions. I.e., the sum of weights with this other shard is higher than the sum of the current intra-shard edges. We could add an additional threshold for that (the difference is more than X) so we avoid too frequent state migration. 


Just use Louvain (iteratively), but used best fit first only the first time - then use dynamic migration to assign groups to shards. 


==> sections/questions.tex <==
%!TEX root = ../main.tex
%=========================================================

\section{Research Questions}

\subsection{Random}

\michal{With increased complexity of inter-shard transaction comes higher cost for the users. So users are naturally incentivized to minimize the number of inter-shard transactions. We could use this mechanism and provide an off-chain oracle that user can use to get the optimal placement, but users don't have to obey.}

\michal{Random thought: what if each user automatically has a subcount for each shard -  <user\_addr>@<shard\_id> with seperate balances. Maybe it would be enough to drastically minimize the number of inter-shard transactions. You only have to perform inter-shard transactions if you don't have enough funds in a specific shard. Probably users rarely spend all their money at once, so the money could be split into sub-accounts. \mustafa{Big exchanges and company will likely do this for sure.}}

\michal{We could also optimize the assignment of miners to shards. Also users with high mining power, could be validators in multiple shards. If that's the case, we should assign them to shards that communicate often. Like that we minimize the cost of inter-shards transactions. \mustafa{Why would that minimise the cost of inter-shard transactions? Worth thinking about full nodes in shards too verifying the chain for themselves.}}


\subsection{Splitting State}
How to decide where to put a new user/utxo? When and where to migrate them?
\begin{itemize}
 \item The clustering method used in the introduction can be modified for dynamic graphs~\cite{aynaud2010static}. We can modify the algorithm and then apply it to the blockchain history to see if it still significantly reduces inter-shard transactions
 \item Facebook uses a similar technique for clustering their state on the fly~\cite{shalita2016social}. Their algorithm for clustering is fairly simple and can be easily implemented. 
\end{itemize}


\subsection{State Management/Resolution}
Once we know how to efficiently split and migrate state, the questions is - how to enforce it?
\begin{itemize}
 \item The cost of the transactions could be dependent on the number of the involved shards. It would automatically incentivize users to put transactions in optimal shards
 \item the state splitting algorithm could be also run by the shards, that will automatically migrate state between them under certain conditions. s
\end{itemize}


\begin{itemize}
 \item How to perform resolution? RapidChain uses TXID to set transaction hash to fall within a specific shard. We could also simply put shard number in the transaction. It should be easy in UTXO, we don't migrate objects, but create a new ones with new shardID/TXID. However, how about account-based? If an account is in shardA and later is migrated into shardB, we'll need a resolution system
 \item Smart sharding must still keep a balance between shards (they should all receive a similar amount of transactions/shards). How to encorce it?
 \item Could smart sharding be used by malicious users?
\end{itemize}


Validators - parts of several shards, and then we reduce the cost of intrashards. The algorithm moves some validators between shards to. Maybe we can ``merge'' shards 

From which threshold is it better to split a shard. In terms of the number of validators. If there are more than a threshold 

Focus on killer apps. 

Validator is a unit of state. 


\subsection{Fees}
How to make sure that all the miners are inceitivized to migrate state? As a miner in an overloaded shard, it might be actually good for me to keep as many users as possible. This would increase the fees offered by the users and I can keep pending transactions ``for later''. 

\section{From the intro}





\begin{itemize}
 \item But there's a problem, when a transaction modifies state in different shards
 \item In the account-based model, this happens when account balances of sender and receiver are in different shards \mustafa{What about for generic smart contracts? Cross-shard transactions can be generalised to involve reading/writing state from multiple shard, which require a lock. Or are you only focusing on payments for now?}
 \item In the UTXO model, this happens when transaction inputs are in different shards than the one processing the transaction

 \item To the best of our knowledge, all the sharding systems use consistent hashing to divide state among shard \mustafa{Ethereum and Chainspace let the user/smart contract developer pick which shard their object goes in!}
 \item This is simple, but causes a lot of inter-shard transactions
 \item And this number grows with the number of shards\mustafa{Depends on object->shard assignment mechanism. If it's random then yeah.}
 \item Blockchains transactions follow patterns observable in social networks. There are group of nodes that communicate a lot between them.
 \item To illustrate this, we take a graph clustering algorithm from social network~\cite{blondel2008fast} and apply it to transaction in Ethereum Rinkeby Testnet.
 \item \Cref{fig:bound} shows that by placing nodes that correlated state (i.e., user that often pay each other), we can almost entirely eliminate inter-shard transaction.\footnote{The clustering was applied to a complete blockchain history. So this is upper-bound - potential baseline for later.}
 \item This paper: i) shows methods for smart state division in blockchain ii)apply them to blockchain in a secure manner
 Note that this comes at a cost: the reasons why people use hashing to attribute objects to shards is because there is often a "killer app"; eg. the coin contract. This means that shards handling killer apps will handle themselves almost 90\% of the traffic, while the other will only handle 10\%.\mustafa{You can say that you are sharding objects, rather than contracts. However Ethereum 2.0 only shards contracts but they use a trick where contracts can spawn contracts, thus each object can get its own contract.} This will then break scalability (or security)
\alberto{Chainspace (in its original version, the NDSS paper) don't exactly use hashes; it relies on $function /phi(object\_id) -> shard$. This function is defined by the smart contract that handle the object, but poorly discuss the tradeoff I mentioned above. Then for implementation, Chainspace uses $\phi = SHA-256$. The technique you describe in the paper is very interesting actually; and could go even further it could use your clustering technique handle the tradeoff between 1/ not localizing killer apps on a single shard and 2/ not use hash. The point is; all papers assume that each shard is of the same size, you could actually use your technique to vary the size of the shard and decide when to split a big shard into two smaller shards, depending on the load then, there is an interesting discussion in considering strong identity (like Omniledger); ie. 1 node = 1 public key; versus a distribution of stake ie. one node may have multiple pk.
Last note; the first Chainspace paper briefly mention that shards can overlap to minimize the impact of the cross-shard transactions VS not localizing killer apps into a single shard -- this could be explored much with your technique
}
\end{itemize}



\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{img/bound}
\caption{Comparison of smart sharding vs consistent hashing in account-based and UTXO}
\label{fig:bound}
\end{figure}



==> sections/simulations.tex <==
%!TEX root = ../main.tex
%=========================================================

\section{Simulations}

Paramiters:
\begin{itemize}
 \item mutiplier for power (how costly are inter-shard transactions
 \item fading multiplier (how dynamic is the network, if everything is random, we should take into account only the most recent transactions)
\end{itemize}





